Clustering multilayer graphs with missing nodes

Relationship between agents can be conveniently represented by graphs. When these relationships have different modalities, they are better modelled by multilayer graphs where each layer is associated with one modality. Such graphs arise naturally in many contexts including biological and social networks. Clustering is a fundamental problem in network analysis where the goal is to regroup nodes with similar connectivity profiles. In the past decade, various clustering methods have been extended from the unilayer setting to multilayer graphs in order to incorporate the information provided by each layer. While most existing works assume - rather restrictively - that all layers share the same set of nodes, we propose a new framework that allows for layers to be defined on different sets of nodes. In particular, the nodes not recorded in a layer are treated as missing. Within this paradigm, we investigate several generalizations of well-known clustering methods in the complete setting to the incomplete one and prove some consistency results under the Multi-Layer Stochastic Block Model assumption. Our theoretical results are complemented by thorough numerical comparisons between our proposed algorithms on synthetic data, and also on real datasets, thus highlighting the promising behaviour of our methods in various settings.

==> Clustering graphs with missing nodes [v2]/aggregate_spectr.tex <==
\subsection{Aggregate spectral Kernel : the complete case}
This method was proposed in \cite{paul2020} without theoretical guarantees. The principle is the following. For each layer $l$ we compute $\hat{U}_K^{(l)}$ the matrix formed by the eigenvectors of $A^{(l)}$ corresponding to the top $K$ singular values. Then we compute $\Tilde{U}_K$ the matrix formed by the top $K$ eigenvectors of the sum $\sum_l \hat{U}_K^{(l)}(\hat{U}_K^{(l)})^T $ and perform $k$-means on the rows of $\Tilde{U}_K$.
So we compute the best $K$-rank subspace associated with each layer and then find the $K$-rank subspace that is the closest to all these subspaces. A similar approach has been used in the context of distributed PCA \cite{fan2019}.



\subsection{Aggregate spectral Kernel : the missing nodes case}

==> Clustering graphs with missing nodes [v2]/conclusion.tex <==
\section{Future work} \label{sec:rel_fut_work}
%
Our theorems require different conditions for consistency (each layer has to be informative enough for Algorithm \ref{alg:k-pod} and $L$ has to be large for Algorithm \ref{alg:sum_of_adj0}). It would be interesting to gain a better understanding of the fundamental limit of clustering with missing nodes. \gb{In this regard the use of two-round algorithms (see for e.g., \cite{AbbeSBM}) that do local refinement after having found a global partition could improve the misclustering rate.
It would also be interesting to consider model-based approaches by considering variational methods (\cite{daudin2008}) or Stochastic-EM algorithms (\cite{celeux1996stochastic}). } 
%\hemant{Add at least one reference each for local refinement, variational methods/ stochastic EM methods.}

We assumed for simplicity that the nodes are missing under a Bernoulli sampling scheme, but other missing patterns could be considered. 
Another important direction would be to relax the strong condition imposed by MLSBM that all layers share the same common partition. For example, it would be more realistic to assume that the partition of networks evolving over time also evolves slowly.

==> Clustering graphs with missing nodes [v2]/early_fusion.tex <==
\section{Early fusion methods: spectral clustering on sum of adjacency matrices} \label{sec:early_fusion}
%\gb{Section 3,4,5 have roughly the same structure, first we motivate the methods by quoting results from the complete setting and then propose an extension to the missing nodes data setting. Shouldn't we start each Section with a subsection "complete data setting" ?}
%
%
Late fusion methods rely heavily on the quality of each layer. However, by  simultaneously using all the information contained in all layers, the clustering performance can be improved in some settings (see the numerical experiments in \cite{paul2020} or \cite{airoldi2014}).
%\hemant{(Is this true that it can be improved?)}
One way to do this is to aggregate the information across layers and then apply a suitable clustering method. This approach will be referred to as an early fusion method.
One simple but popular way to do this is to take the mean of the adjacency matrices (see for e.g., \cite{Bhattacharyya2018SpectralCF, paul2020}). Then, the $k$-means algorithm can be applied to the rows of the $n \times K$ eigenvector matrix associated with the top $K$ eigenvalues (in absolute value) of  $A = L^{-1} \sum_l A^{(l)}$.

\subsection{Imputing missing entries with zeros} \label{subsec:early_fusion_impute_zero}
%\paragraph{Complete data setting.} 
%\paragraph{Extension to missing data setting.} 
A natural way to extend the aforementioned approach to the setting of missing nodes is to fill the missing entries with zeros, thus leading to Algorithm \ref{alg:sum_of_adj0}. \gb{The worst-case complexity of the algorithm is $O((L+K)n^2)$.}
%This will create a bias since it is equivalent to considering the missing nodes as nodes with no relations to the other. In order to reduce this bias we also propose an iterative way to impute missing value leading to Algorithm \ref{alg:sum_of_adj_c}. 
%First let's introduce some notation and describe the algorithm \ref{alg:sum_of_adj0}.
%
%
\begin{algorithm}[!ht]
\caption{Sum of adjacency matrices with missing entries filled with zeros}\label{alg:sum_of_adj0}
\begin{flushleft}
        \textbf{Input:} The number of communities $K$, the matrices $A^{(l)}$ and $\Omega^{(l)}$.
\end{flushleft}
\begin{algorithmic}[1]
\State Compute $A=L^{-1}\sum_lA^{(l)}\odot \Omega^{(l)}$.

\State Compute the eigenvectors $u_1, \ldots, u_K$ associated with the $K$ largest eigenvalues of $A$ (ordered in absolute values) and form $U_K = [u_1 \ u_2 \ \cdots \ u_K]$.

\State Apply $K$-means on the rows of $U_K$ to obtain a partition of $\calN$ into $K$ communities.
\end{algorithmic}
%
%
\textbf{Output:} A partition of the nodes $\calN =\cup_{i=1}^K \calC_i$.
\end{algorithm}
%
%
%

Let us denote  $\Tilde{A}=\rho^{-2}L^{-1}\sum_l A^{(l)}\odot \Omega^{(l)}$ (clustering on $A$ or $\Tilde{A}$ is equivalent since the two matrices are proportional, but for the analysis it is more convenient to work with $\Tilde{A}$). Clearly $\expec(\Tilde{A})=L^{-1}\sum_l \expec(A^{(l)})$ (since the diagonal entries of $A^{(l)}$ are zero). Denote by $\expec(X|\Omega)$ to be the expectation of $X$ conditionally on $\Omega=(\Omega^{(1)}, \ldots, \Omega^{(L)})$ and 
%let $\delta$ denote $|\lambda_{K+1}(\tilde{A})-\lambda_K(\expec(\tilde{A}))|$ where $\lambda_k(B)$ is the $k$th largest singular value of $B$.
let $\lambda_K$ denote the $K$th largest singular value of $\expec(\Tilde{A})$.
We have $\expec(\Tilde{A}| \Omega)=\rho^{-2}L^{-1}\sum_l \expec(A^{(l)})\odot \Omega^{(l)}$.
Using the same kind of perturbation arguments and concentration inequalities as in~\cite{lei2015}, we can relate $\tilde{A}$ to  $\expec(\Tilde{A}| \Omega)$ and then use Bernstein inequality to relate $\expec(\Tilde{A}| \Omega)$ with  $\expec(\Tilde{A})$. This leads to the following bound on the misclustering rate.
% 
%
\gb{
\begin{theorem}
\label{thm:sumadj}
 Under the missing nodes MLSBM in Section \ref{subsec:missing_node_MLSBM}, there exist constants $C_0, C_1 > 0$ such that with probability at least $1-O(n^{-1})$, the solution $\hat{Z} \in \mathcal{M}_{n,K}$ obtained from Algorithm \ref{alg:sum_of_adj0} satisfies
%
%
\begin{align*}
&r(\hat{Z},Z)\leq \underbrace{\frac{C_0K}{\rho ^4\lambda_K^2}\left(\frac{np_{max}}{L}+\frac{\log n }{L}\right)}_\text{noise error}+\\
&  \underbrace{C_1K\frac{(\rho^{-2}-1)^2}{\lambda_K^2} \left((np_{max})^2\frac{\log(n)}{L} +
\left(\frac{np_{max} \log n}{L}\right)^2 \right)}_\text{missing data error}.
%
%
\end{align*}
%        
%
\end{theorem}
}
% 
%
If $L$ is small then the missing data error could be larger than one making the upper bound  trivial. In the best case scenario, we expect that $\lambda_K$ scales as $np_{max}$. So we need at least $C\log n$ layers to get a non trivial upper bound. In order to obtain asymptotic consistency, it is necessary that $L\gg \log n$.
However, experiments show that even when $L$ is small, Algorithm \ref{alg:sum_of_adj0} gives good results as long as the layers are dense enough and the number of missing nodes is not too large.

%\gb{comparison added }
When $\rho=1$ and $np_{max}\geq \log n$  the upper bound becomes $O((Lnp_{max})^{-1/2})$ thus matching the bound obtained by \cite{Bhattacharyya2018SpectralCF} in a more general regime. See the supplementary material for other comparisons.

%\hemant{(Isn't the following text not relevant now since it refers to the refined analysis?)} In the following section we are going to show that in the symmetric SBM setting even the distance between the eigenvectors of $\expec(\Tilde{A}| \Omega)$ and $\expec(\Tilde{A})$ is not small, the sign of the entries of the second eigenvector of $\expec(\Tilde{A}| \Omega)$ allows to recover the communities until $\rho$ and the eigenvalues of the matrices $A^{(l)}$ satisfy one condition. This explains why the algorithm succeeds even when the number of layer is inferior to $\log n$ and also why the performance of the algorithm worsens dramatically under some threshold on $\rho$.
%
%  
\subsection{Iteratively imputing the missing entries} \label{subsec:early_fusion_impute_iter}
%\hemant{This still needs rewriting...}
When the number of missing nodes is important, filling missing entries with zero can lead to a huge bias and hence poor clustering performances. In order to reduce the bias we propose an alternative way of imputing the missing values (outlined as Algorithm \ref{alg:sum_of_adj_c}) based on the fact that each adjacency matrix is a noisy realization of a structured matrix. 

At iteration $t$, given an initial estimate $\hat{U}_K^{t} \in \mathbb{R}^{n\times K}$ of the common subspace we can estimate the membership matrix $\hat{Z}^t$ by applying $k$-means on  $\hat{U}_K^{t}$. Then, we can estimate the connectivity matrix $\hat{\Pi}^{(l),t}$ for each $l$ as
%
\begin{equation}\label{eq:sum_of_adj_c}
    \hat{\Pi}^{(l),t}=((\hat{Z}^t)^T\hat{Z}^t)^{-1}(\hat{Z}^t)^TA^{(l),t}\hat{Z}^t((\hat{Z}^t)^T\hat{Z}^t)^{-1}.
\end{equation}
%
Given $\hat{Z}^t$ and  $\hat{\Pi}^{(l),t}$ we estimate the rows and columns corresponding to missing nodes. Indeed, the connectivity profile of a node $i$ in layer $l$ is given by the $i$th row of $\hat{Z}^t\hat{\Pi}^{(l),t}(\hat{Z}^{t})^{T}$. By replacing the rows and columns of missing nodes by their estimated profiles, and leaving the value of observed nodes unchanged, we obtain the updated imputed matrix $A^{(l),t+1}$. Applying spectral clustering on $L^{-1}\sum_l A^{(l),t+1}$ then leads to an updated estimate $\hat{U}_K^{t+1}$ of the common subspace.  The procedure can be repeated using $\hat{U}_K^{t+1}$ and $A^{(l),t+1}$, thus iteratively imputing the missing values in order to obtain ``completed'' adjacency matrices that share the same $K$ rank structure across layers. \gb{In the worst case, the complexity of the algorithm run with $T$ iterations is $O((K+L)n^2 T+LKnT)$.} 
%
%\hemant{Where in Algorithm \ref{alg:sum_of_adj_c} is there a sum of adjacencies? You also need to explain some of the steps in the algorithm, this part is woefully lacking detail at the moment.}

Similar iterative imputation methods have been studied in the context of principal component analysis, see for e.g., \cite{hetePCA, primePCA}.
%
%
\begin{algorithm}[!ht]
\caption{Sum of adjacency matrices with missing entries filled iteratively}\label{alg:sum_of_adj_c}
%
\begin{flushleft}
        \textbf{Input:} Number of communities $K$; $J_l$ and $A_{J_l}\in \mathbb{R}^{n\times n}$ for each $l$; initial estimate of the common subspace $\hat{U}_K^{0}\in \mathbb{R}^{n\times K}$ (with orthonormal columns)    obtained from Algorithm \ref{alg:sum_of_adj0}; number of iterations $T$.
\end{flushleft}
%
\begin{algorithmic}[1]
\State Initialize $t=0$ and $A^{(l), 0}=A_{J_l}$ for all $l$.
\Repeat 
\State Given $\hat{U}_K^{t}$, estimate the membership matrix $\hat{Z}^t$ and the connectivity parameters $\hat{\Pi}^{(l),t}$ for all $l$ by using \eqref{eq:sum_of_adj_c}.

\State For each $l$, replace rows (and corresponding columns) of $A^{(l)}$ corresponding to a missing node $i$ by the $i$th row of $\hat{Z}^t\hat{\Pi}^{(l),t}\hat{Z}^{t^T}$ to form  $A^{(l),t+1}$.

\State Compute the eigenvector matrix $\hat{U}_K^{t+1} = [u_1^{t+1} \ u_2^{t+1} \  \cdots \ u_K^{t+1}]$  associated with the $K$ largest (in absolute order) eigenvalues of $L^{-1}\sum_l A^{(l),t+1}$. Update $t\leftarrow t+1$.

\Until{$t\leq T$} 
\State Apply $K$-means on $\hat{U}_K^{T}$ to get a partition of $\calN$.
\end{algorithmic}
% 
\textbf{Output:} A partition of the nodes $\calN =\cup_{i=1}^K \calC_i$.
\end{algorithm}
%
%
In our experiments, Algorithm \ref{alg:sum_of_adj_c} is seen to perform significantly better than other methods when $\rho$ decreases. While we do not currently have any statistical performance guarantee for Algorithm \ref{alg:sum_of_adj_c}, establishing this is an interesting direction for future work.

==> Clustering graphs with missing nodes [v2]/experiments.tex <==
\section{Numerical experiments} \label{sec:num_exps}
\subsection{Synthetic data} \label{subsec:num_syn_exps}
%
% 
We now describe simulation results when the multilayer graph is generated from the missing nodes MLSBM. The normalized mutual information (NMI) criterion is used to compare the estimated community to the ground truth partition. It is an information theoretic measure of similarity taking values in $[0,1]$, with $1$ denoting a perfect match, and $0$ denoting completely independent partitions. Nodes that are not observed at least once are removed. 
The diagonal (resp. off-diagonal) entries of the connectivity matrices are generated uniformly at random over $[0.18,0.19]$ (resp. $0.7*[0.18,0.19]$). The ground truth partition is generated from a multinomial law with parameters $1/K$. While $K=3$ is fixed throughout, the parameters $n,\rho$ and $L$ are varied suitably. The average NMI is reported over $20$ Monte Carlo trials. As shorthand, we denote Alg. \ref{alg:k-pod} by \kpod, Alg. \ref{alg:sum_of_adj0} by \sumadjz, Alg. \ref{alg:sum_of_adj_c} by \sumadji, and \eqref{olmf:miss_def} by \olmfm.
 
% The OLMF estimator is computated with a BFGS algorithm similar to the one described in \cite{paul2020}. We however relaxed the constraint that the gradient remains on the Stiefel manifold of $K$-orthogonal matrices in $\mathbb{R}^{n\times n}$. We initialize the parameters with the values obtain by clustering the sum of adjacency matrices.
 
Figure \ref{plot_rho} shows that \sumadjz~ gives good results unless $\rho$ is too small. Then, the performance of this method decreases quickly. This suggests that there is a threshold involving $\rho$ and the difference between intra and inter connectivity parameters. Figure \ref{plot_n} supports this claim. When $\rho$ is small, the performance of \sumadjz~doesn't improve when $n$ increases. So even if the separation between communities improves, the intra and inter connectivity parameters remain the same suggesting a link between these parameters and  $\rho$.
 
When $L$ increases (see Figs. \ref{plot_rho} and \ref{plot_L}), the performance of all methods improves. However, performance of \kpod~  improves less quickly than other methods. This is expected since contrary to other methods, \kpod~ relies more on the quality of each individual layer. 
\olmfm~ and \sumadji~ exhibit better performance than others in the challenging situation when $\rho$ is small, and perform as well as the others when $\rho \approx 1$. They  perform significantly better than \kpod, especially when $L$ is large.
 %\gb{The title inside the plot "L=4,K=3,n=..." can be moved within the plot area to save space}
  \begin{figure}[!ht]
  \center
   \includegraphics[scale=0.37]{images/plot_rho2.png}
   \caption{   NMI vs $\rho$ for different values of $L$}
   \label{plot_rho}
\end{figure}


 
 \begin{figure}[!ht]
 \center
   \includegraphics[scale=0.37]{images/plot_L2.png}
     \caption{ NMI vs $L$ for different values of $\rho$}
     \label{plot_L} 
\end{figure}
 

 \begin{figure}[!ht]
 \center
   \includegraphics[scale=0.37]{images/plot_n2.png}
     \caption{  NMI vs $n$ for different values of $\rho$}
     \label{plot_n}
\end{figure}
%

\subsection{MIT Reality Mining dataset} \label{subsec:mit_mining_exps}
This dataset records interactions (measured by cell phones activities) between $96$ students and staff at MIT in the 2004-05 school year (see \cite{mit}). We used the dataset as provided by the R package `GreedySTBM'.  As in \cite{airoldi2014} we removed the first and last layers, then discretized the time into one week intervals. The number of times two persons had an interaction during the week is not conserved in order to have a simple undirected graph corresponding to each layer. In total we obtained $32$ layers. 
For different values of $\rho$, we randomly removed nodes in each layer of the multilayer network. The average NMI over $50$ Monte Carlo trials is reported in Table \ref{table:mit} for our methods. The ground truth partition here is taken to be that obtained from \sumadjz~ when $\rho=1$. 
%\gb{We can present the results with plots instead of table, but I'm not sure it will help to save space.}
\begin{table}[!ht]
\centering
\begin{tabular}{rrrr}
  \hline
 $\rho$ & \sumadjz & \olmfm & \sumadji \\ 
  \hline
  1 & 1.00 & 1.00 & 1.00 \\ 
  0.9 & 0.99 & 0.96 & 0.99 \\ 
  0.8 & 0.97 & 0.86 & 0.97 \\ 
  0.7 & 0.96 & 0.93 & 0.96 \\ 
  0.6 & 0.94 & 0.79 & 0.94 \\
  0.5 & 0.89 & 0.91 & 0.90 \\
  0.4 & 0.76 & 0.73 & 0.78 \\
  0.3 & 0.56 & 0.57 & 0.62 \\
  0.2 & 0.26 & 0.41 & 0.36 \\
  0.1 & 0.09 & 0.10 & 0.11 \\ 
   \hline
\end{tabular}
\caption{NMI vs $\rho$ for MIT Reality Mining dataset}
\label{table:mit}
\end{table}
%
%
We disregarded \kpod~ because even when $\rho = 1$, its performance was disappointing and very sensitive to the initialization. This is not very surprising since this method works only if each layer is informative enough while we have a multilayer network where individual layers can be very sparse.

The performance of the other three methods studied are quite similar when $\rho$ is not too small ($\rho \geq 0.4$). However, the performance of \olmfm~ seems to be quite sensitive to initialization since for $\rho \in \set{0.6,0.8}$ its performance is worse than \sumadjz~ and \sumadji. Even if we remove half of the nodes in each layer we can still approximately recover the partition. 

\subsection{Malaria parasite genes network} \label{subsec:malaria_parasite_exps}
The dataset was constituted by \cite{malaria} to study the var genes parasite Plasmodium falciparum involved in Malaria. 
%These var genes are characterized by their high rate of recombination. 
%precluding the use of traditional phylogenetic tools. 
The nodes of the dataset correspond to $307$ different amino acid sequences and each of the $9$ layers corresponds to a highly variable region (HVR). Two nodes are linked in a given layer if there is a common block sequence between the corresponding amino acid sequences within the HVR associated to the layer. The analysis in \cite{malaria} and \cite{regtens} shows that the first six layers share the same community structure with $K=4$. Hence we restrict our study to the first six layers with $K=4$. We use the same procedure as before to delete nodes and to select the ground truth partition. \kpod~ was disregarded for the same reason as the previous experiment.
%
%
\begin{table}[!ht]
\centering 
\begin{tabular}{rrrrr}
  \hline
  $\rho$ & \sumadjz & \olmfm & \sumadji \\ 
  \hline
  1 & 1.00  & 0.99 & 1.00 \\ 
  0.9 & 0.75 & 0.75 & 0.72 \\ 
  0.8 & 0.63 & 0.62 & 0.58 \\ 
  0.7 & 0.47 & 0.49 & 0.47 \\ 
  0.6 & 0.32 & 0.37 & 0.34 \\ 
  0.5 & 0.22 & 0.20 & 0.26 \\ 
  0.4 & 0.13 & 0.07 & 0.16 \\
   \hline
\end{tabular}
\caption{NMI vs $\rho$ for Malaria parasite genes network}
\label{table:malaria}
\end{table}
%
%
As $\rho$ decreases, the clustering performance decreases rapidly due to a weak separation between the clusters as shown in Table \ref{table:malaria}. 


==> Clustering graphs with missing nodes [v2]/intermediate_fusion.tex <==
\section{Intermediate fusion methods: OLMF estimator} \label{sec:inter_fusion_olmf} 
%
Orthogonal linked matrix factorization (OLMF) is a clustering method for multilayer graphs that originated in the work of \cite{dhillon} in the complete data setup, and was later analysed in \cite{paul2020}. It shows good performance in various settings and outperforms spectral clustering when the multilayer network contains homophilic and heterophilic communities (see the numerical experiments in \cite{paul2020}). 
%\hemant{Is this shown in Paul and Chen experiments? You should always support such claims with appropriate citation.}
%

\subsection{The complete data setting} \label{subsec:olmf_complete}
In the complete data setting, the OLMF estimator is a solution of the following optimization problem 
%
\begin{equation}\label{eq:Olmf}
    (\hat{Q}, \hat{B}^{(1)}, \ldots , \hat{B}^{(L)}) \in \argmin{\substack{Q^TQ=I_k\\B^{(1)}, \ldots, B^{(L)}} }\sum_l|| A^{(l)}-QB^{(l)}Q^T||_F^2,
\end{equation} 
%
where $Q\in \mathbb{R}^{n\times K}$,  $B^{(l)}\in \mathbb{R}^{K\times K}$. Note that there is no constraint on the values taken by the entries of $B^{(l)}$.
%This optimization problem can be considered as a relaxation of the following least square estimator studied in~\cite{jinLei2019} : \begin{equation}\label{eq:lsMlsbm}(\hat{z}, \hat{B}^{(1)}, \ldots , \hat{B}^{(L)})\in \argmin{z, B^{(1)}, \ldots , B^{(L)}}\sum_l \sum_{i\neq j}(A^{(l)}_{ij}-B^{(l)}_{z(i)z(j)})^2\end{equation}  where $z\in [K]^n$ is a possible assignment of the communities and $B^{(l)}\in \mathbf{R}^{K\times K}$. Since every such $z$ can be bijectively associated with a membership matrix $Z\in \calM_{n,K}$, the optimization problem \eqref{eq:lsMlsbm} is equivalent to

%\begin{equation}
%\label{eq:lsMlsbm2}   (\hat{Z}, \hat{B}^{(1)}, \ldots , \hat{B}^{(L)}) \in \argmin{Z, B^{(1)}, \ldots , B^{(L)}} \sum_l||A^{(l)}-ZB^{(l)}Z^T ||^2_F,\end{equation}
%where $Z\in \calM_{n,K}$ and $B^{(l)}\in \mathbb{R}^{K\times K}$. If we relax the constraint $Z\in \calM_{n,K}$ to $Z^TZ=I$ we obtain \eqref{eq:Olmf}.

A little algebra (see \cite{paul2020}) shows that the optimization problem \eqref{eq:Olmf} is equivalent to 
%
\begin{equation}\label{eq:Olmf2}
    \hat{Q}\in \argmax{Q^TQ=I_k}\sum_l||Q^TA^{(l)}Q||_F^2,\quad  \hat{B}^{(l)}=\hat{Q}^TA^{(l)}\hat{Q}
\end{equation}
%
for $l=1,\dots,L$. The OLMF estimator can be computed with a gradient descent on the Stiefel manifold (see \cite{paul2020} and supplementary material therein). The community estimation is then obtained by applying $K$-means on the rows of $\hat{Q}$. 

\subsection{Extension to the missing nodes setting} \label{subsec:olmf_missing}
%
%
We now present an extension of the OLMF estimator to the setting of missing nodes. By replacing the matrices $A^{(l)}$, $Q$ in the objective function in \eqref{eq:Olmf} with $A_{J_l} \in \mathbb{R}^{n \times n}$, $Q_{J_l} \in \mathbb{R}^{n \times K}$, we end up with the following modification for the incomplete setting
%, $A_{J_l}$ (resp. $Q_{J_l}$) denote the matrix obtained from $A$ (resp. $Q$) \hemant{($A$ should be $A^{(l)}$ right?)} by replacing rows and columns (resp. rows) whose index don't belong to $J_l$ by zeros. Depending on the context, $A_{J_l}$ (resp. $Q_{J_l}$) can also denote the matrix of size $|J_l|\times |J_l|$ (resp.  $|J_l|\times K$) where row and column indices (resp. row indices) not lying in $J_l$ are removed.

%Consider the optimization problem \hemant{Below you use $B^{(l)}$ but above its $B^{l}$}
%
\begin{equation}\label{olmf:miss_def}
      (\hat{Q}, \hat{B}^{(1)}, \ldots , \hat{B}^{(L)})\in \argmin{\substack{Q^TQ=I_k\\B^{(1)}, \ldots, B^{(l)}}}\sum_l|| A_{J_l}-Q_{J_l}B^{(l)}Q_{J_l}^T||_F^2. 
\end{equation} 
%
%
In our experiments, we employ a BFGS algorithm for solving \eqref{olmf:miss_def}. \gb{The worst-case complexity of the algorithm is $O(LK(n^2+Kn))$.} Denoting the objective function in \eqref{eq:Olmf2} by $F$, its gradients are given by 
%
\begin{align*} 
\frac{\partial F}{\partial Q}&=-2\sum_l(A_{J_l}-Q_{J_l}B^{(l)}Q_{J_l}^T)Q_{J_l}B^{(l)}, \\
%
\frac{\partial F}{\partial B^{(l)}}&=-Q_{J_l}^T(A_{J_l}-Q_{J_l}B^{(l)}Q_{J_l}^T)Q_{J_l}.
\end{align*}
%
We relax the constraint that the gradient remains on the Stiefel manifold of $n \times k$ matrices, and  initialize the parameters using Algorithm \ref{alg:sum_of_adj0}.
%

The optimization problem in \eqref{eq:Olmf2} can be motivated via the missing nodes MLSBM as follows. If we replace the noisy realization $A_{J_l}$ with  $(Z\Pi^{(l)}Z^T)\odot \Omega^{(l)} $ then one can show (under some conditions) that the solution $\hat{Q}$
%\hemant{should this be $\hat{Q}$ as written later below? But in the proposition you use $Q$..} 
%\gb{I replaced $Q$ by $\hat{Q}$}
of \eqref{olmf:miss_def} has the same column span as the ground truth $Z \in \mathcal{M}_{n,K}$. This is shown formally in the following proposition.  
%\hemant{the latter matrix does not have $0$s on the diagonal. But $A_{J_l}$ does have $0$s on the diagonal.}
%\gb{Indeed, but it is more difficult to prove something in this case. Paul and Chen also avoid this situation. The zero diagonal can be considered as censure from $(Z\Pi^{(l)}Z^T)$ that are the relevant underlying $K$ rank bl0ock matrices.}
%
%
\begin{proposition} \label{prop:olmf}
Assume that $\Pi^{(l)}$ is full rank for each $l$, and that for each $l, l'$ the sets $J_l\cap J_{l'}$ intersect all communities. Then if $A_{J_l}=(Z\Pi^{(l)}Z^T)\odot \Omega^{(l)}$, it holds that the solution of \eqref{olmf:miss_def} is  given by $\hat{Q}=Z(Z^TZ)^{-1/2}$ and $\hat{B}^{(l)}=(Z^TZ)^{1/2}\Pi^{(l)}(Z^TZ)^{1/2}$ and is unique up to an orthogonal transformation. Moreover if $i$, $j$ belong to the same community, then $\hat{Q}_{i*}=\hat{Q}_{j*}$.
\end{proposition}

%
%\hemant{add remark/text explaining the bias due to zeros on the diagonal of the adjacency.}
The matrix $\expec(A^{(l)})$ can be considered as a slight perturbation of $Z\Pi^{(l)}Z^T$ 
%(the underlying rank $K$ matrix encoding the signal) 
since the former has zeros on the diagonal. Thus the proposition shows that when there is no noise, the column-span of $\hat{Q}$ (the solution of \eqref{olmf:miss_def}) is the same as the ground truth partition $Z$.

==> Clustering graphs with missing nodes [v2]/intro.tex <==
\section{Introduction}

%--- Background on unilayer graphs ----%
Graphs are a powerful tool to represent relationships between agents. Due to applications in a wide array of fields including biology, sociology, ecology and economics (see for e.g., \cite{brain, airoldi2014,kivela_eco, Kim2015}), the analysis of networks has received significant interest over the last two decades. One fundamental problem of network analysis is \emph{clustering} which involves detecting communities by regrouping nodes having similar connectivity properties. Numerous clustering algorithms have been developed over the years based on different approaches such as modularity maximization, maximum likelihood, random walks, semi-definite programming and spectral clustering (see for instance the survey articles by \cite{fortunato2010} and \cite{AbbeSBM}).

%---- Motivations for multilayer graphs ---%

 Often, relationships are better understood through different modalities. These multiple aspects of relationships can be represented by a multilayer graph where each layer is a graph representing the interactions between agents for one modality. For e.g., social interaction between a set of people can be recorded via email exchanges, phone calls, professional links, and so on. Each level of interaction can be encoded into a simple graph and the collection of these graphs leads to a multilayer representation. Another important example of a multilayer graph is given by a  time-varying network where each view of the network at a given time corresponds to a different layer.

%---- Brief summary of existing works related to multilayer graphs clustering ---%
 Over the last decade, many methods have been proposed for clustering multilayer graphs such as those based on matrix factorization, spectral methods, maximisation of a modularity function or probability model-based approaches; see \cite{Kim2015} for a survey. Consistency results for the recovery of the partition under a stochastic generative model have also been shown for some algorithms, see for example \cite{paul2020}, \cite{pensky2019}, \cite{lei2020tail} and \cite{Bhattacharyya2018SpectralCF}. 
 %\hemant{I think there are still sufficiently many results no? They should be cited here and we should have a related work section towards the end where we discuss those technical results.} 
% \gb{I added references for consistency results for partition recovery under MLSBM or dSBM like models. Maybe it is not an exhaustive list.}

Most existing approaches assume that all the layers share the same set of nodes. In practice, however, data are often incomplete; in particular, the set of observed nodes can clearly vary across layers. For example, in social networks evolving over time, the set of nodes can change due to people leaving/joining the network. This is the setting considered in the present paper.
%\gb{Maybe we should emphasize in the introduction that missing nodes are more difficult to handle than missing edges and give references for missing edges ?}
%--- Incomplete multi-view clustering ---%

\subsection{Related work} 


%\footnote{Multi view data arises when different sets of features are available for each individual object. Multilayer graphs can be considered as a particular case of multi view data.}
%\hemant{does this mean that these papers consider a stochastic generative model but do not show consistency results for recovering the clustering? I think they do show some kind of theoretical result (generalization bound for example) so this needs to be specified}
%Our framework is more specific but we provide some theoretical guarantees in terms of bounds on the misclustering rate. Moreover, contrary to the algorithms proposed in the previous works in IMVC, our proposed methods do not rely on the choice of tuning parameters. Nevertheless, there are common ideas underlying the design of all these algorithms.

\paragraph{Clustering on multi-layer graphs. } As noted by \cite{paul2020}, clustering strategies for multilayer graphs can be roughly categorized into three groups: {\bf early fusion} methods where all views are aggregated and then clustering is performed, {\bf intermediate fusion} methods where the algorithm finds a factor common to all the views, and {\bf final aggregation} methods where each individual view is processed separately and a consensus partition is formed.  
In the complete setting, different algorithms have been proven to be consistent under a multilayer stochastic block model assumption (see Section \ref{subsec:mlsbm}). Among them are spectral clustering on the sum of adjacency matrices (e.g., \cite{Bhattacharyya2018SpectralCF,paul2020}) or on the sum of squared adjacency matrices with bias correction (e.g., \cite{lei2020tail,bhattacharyya2020general}), orthogonal linked matrix factorization (e.g., \cite{paul2020}), and co-regularized spectral clustering (e.g., \cite{paul2020}). Existing misclustering bounds for these methods are gathered in the supplementary material. 
\gb{
\paragraph{Incomplete Multi-View Clustering (IMVC).}Recently a similar problem has been addressed in the  context of IMVC, see for example \cite{imvc}, \cite{hu2019onepass} and references therein. To the best of our knowledge, no consistency results for the recovery of the ground truth clustering structure are shown in this line of work. Algorithms designed for the IMVC framework cannot be directly applied to our setting since they apply to a collection of feature vectors. However they could possibly be adapted, in a non trivial manner, to our framework. For example, in the complete setting, the OMVC method proposed by \cite{hu2019onepass} can be considered as a variant of the OLMF estimator proposed by \cite{paul2020}  where the optimization problem is modified in order to take into account the symmetry of the inputs. Similarly, if there were no missing views, the algorithm proposed by \cite{imvc} resembles a variant of the co-regularized spectral clustering method of \cite{paul2020} for clustering multilayer graphs. We leave the adaptation of the algorithm proposed by \cite{imvc} to our setting for future work. }

%In recent years, the problem of clustering unilayer networks with missing edges has drawn attention. For e.g., variational inference methods have been proposed for different missing edge patterns in \cite{tabouy2019} and an estimator robust to missing edges and outliers has been studied in \cite{gaucher2019link}. Missing nodes can also be reinterpreted in the missing edges setting where a node is missing when all the connections with other nodes are missing. However, it introduces strong dependencies between the missing connections and the aforementioned approaches are unlikely to generalize to this setting. 
%As argued in the supplementary material, under a Bernoulli sampling scheme, handling missing nodes is far more difficult than handling missing edges. 

%In order to generalize these strategies to the incomplete case, we will also consider imputation methods -- especially for early fusion methods. \hemant{we can remove this last sentence?}

%---Contribution and paper organisation---%
\subsection{Contributions} %\hemant{Needs a bit of rewriting. Mention contributions of Sections 3,4,5,6 as bullets} 
%\gb{Rewritten with bullet}
We consider the problem of clustering multilayer graphs with missing nodes under a Multi-Layer Stochastic Block Model (MLSBM)  described in Section \ref{sec:probsetup}. Our contributions are as follows.
%
%
\begin{itemize}
    \item  In Section \ref{subsec:kpod_fin_agg} we propose a final aggregation method based on a variant of $k$-means for incomplete data (Algorithm \ref{alg:k-pod}), and derive a  bound for the misclustering rate.
    \item  Section \ref{sec:early_fusion}  extends a popular early fusion method -- based on spectral clustering applied to the sum of adjacency matrices -- to the missing nodes setting. Section \ref{subsec:early_fusion_impute_zero} studies this by imputing the missing entries with zeros (Algorithm \ref{alg:sum_of_adj0}), and contains an upper bound for the misclutering rate. Section \ref{subsec:early_fusion_impute_iter} proposes an alternative method (Algorithm \ref{alg:sum_of_adj_c}) wherein the missing entries are imputed iteratively. This method is shown to perform well in our experiments.
    \item  Section  \ref{subsec:olmf_missing} proposes an extension of an intermediate fusion method -- namely the Orthogonal Linked Matrix Factorization (OLMF) method studied by \cite{paul2020} -- to the missing nodes setting.
    \item In Section \ref{sec:num_exps} we empirically evaluate our algorithms on synthetic data, and also on real datasets.
\end{itemize}
%

%-----------------------
% Notations
%-----------------------

%\paragraph{Notations.} 
%\gb{I added the notation [n]}
\subsection{Notations}
The set of integers $\lbrace 1, \ldots, n\rbrace$ will be denoted by $[n]$. For a matrix $M\in \mathbb{R}^{n\times n}$, its Frobenius (resp. operator) norm is denoted by $||M||_F$ (resp.  $||M||$). The notation $M_{i*}$ (resp. $M_{*j}$)  denotes the $i$-th row (resp. $j$-th column) of $M$. For any subset $J$ of $[n]$ and symmetric matrix $M\in \mathbb{R}^{n\times n}$, $M_J \in \mathbb{R}^{|J|\times |J|}$  denotes the square submatrix of $M$ obtained by deleting rows and columns whose index doesn't belong to $J$. For a non symmetric matrix $Z\in \mathbb{R}^{n\times K}$, $Z_{J}$ denotes the submatrix of $Z$ obtained by deleting rows whose index doesn't belong to $J$.
Sometimes, it will also be convenient to consider $A_J$ (resp. $Z_J$) as a $n\times n$ (resp. $n\times K$) matrix where the rows and columns (resp. only the rows) whose index doesn't belong to $J$ are filled with zeros; this will be clear from the context.
$I_n$ denotes the identity matrix of size $n$. Constants will be denoted by the letters $c$ and $C$, eventually indexed by a number to avoid confusion. Within proofs the values of constants can change from line to line whereas they are denoted with the same letter for simplicity.

==> Clustering graphs with missing nodes [v2]/late_fusion.tex <==
\section{Final aggregation methods} \label{sec:fin_agg_methods}
%
A natural way to extend unilayer graph clustering to the multilayer setting is to analyze each layer separately and then find a consensus partition -- such approaches are referred to as final aggregation methods. For example, one can apply any clustering method on each individual layer, take one layer's labels as a reference,  find for each remaining layer the permutation of its labels that maximizes the agreement with the reference layer, and then define a consensus community by majority voting as discussed in \cite{airoldi2014}. 
There exist alternative ways to avoid the cumbersome issue of label switching ambiguity such as the `aggregate spectral kernel' considered in \cite{paul2020}. 
%For example, \cite{paul2020} propose the `aggregate spectral kernel' method that  performs spectral clustering on $L^{-1}\sum_l \hat{U}^{(l)}(\hat{U}^{(l)})^T$ where $\hat{U}^{(l)} \in \mathbb{R}^{n \times K}$ is the eigenvector matrix associated with the largest $K$ eigenvalues (in absolute value) of $A^{(l)}$. 
Such methods rely on the quality of each individual layer and are often empirically outperformed by other methods as shown in \cite{paul2020,airoldi2014}. 

Final aggregation methods are still relevant in the missing nodes context. Indeed, if we have exact recovery for each layer, and if for all $k$ there is at least one common node between two layers belonging to $\calC_k$, then we can easily reconstruct the whole partition even when the set of common nodes is very small. Hence such methods can be considered as baseline methods.  


%The aggregate spectral kernel method can be adapted to the missing node setting by setting $\hat{U}^{(l)}$ as the eigenvector matrix 
%\hemant{there is a problem with this notation, it is not consistent with what is defined in the next section.},
%corresponding to the top $K$ eigenvalues (in absolute value) of $A^{(l)}\odot \Omega^{(l)}$. However, the performance of this method is not satisfactory as shown in Section \ref{sec:num_exps}. So we propose an alternative method which we now describe.\gb{These last two sentences have perhaps to be reconsidered depending on tomorrow experiments. Also, perhaps agrregate spec. clust. should be put as a subsection}
%\gb{Paragraph rewritten}
%\hemant{This para need rewriting for clarity} One way to cluster nodes from a multilayer graph is to perform clustering on each individual layer and then find a consensus partition using majority vote, for example (see \cite{airoldi2014} and the references therein). 
%This method can be efficient in some settings. For instance, if we could exactly recover the partition in each individual layer (when for each $l$, $p_{max}^{(l)}\geq C\log(n_{J_l})/n_{J_l} $), it 
%would be easy to identify labels between %the partitions obtained for each layer %and hence 
%is easy to obtain a consensus community; this is the case even if some nodes are missing.
%In general, however, it can be difficult to identify the community labels between layers. Indeed, when the number of communities increase since there are $K!$ possible permutation of the labels it becomes computationally hard to test all the possible permutation. \hemant{did not understand why $K!$ cases..} In order to avoid this problem, other methods have been proposed in the complete data setting. The general idea is to combine the eigenvectors obtained after applying spectral clustering on each layer instead of using the labels resulting from the $k$-means algorithm applied to the rows of a suitable eigenvector matrix associated with each layer. For example, \cite{paul2020} propose to perform spectral clustering on $L^{-1}\sum_l U_K^{(l)}(U_K^{(l)})^T$ where $U_K^{(l)} \in \mathbb{R}^{n \times k}$ is the matrix formed by the eigenvectors associated with the largest $K$ eigenvalues (in absolute value) of $A^{(l)}$.  \hemant{Rewrite this last part starting from ``For example, ...''}


\subsection{A method based on a variant of $k$-means for incomplete data} \label{subsec:kpod_fin_agg}
%
%
We now propose a final aggregation method for clustering multilayer graphs in the incomplete setting; it avoids the aforementioned label switching problem. 

For each layer $l$, we can compute the matrix $\hat{U}_{J_l}$ of size $|J_l|\times K$ corresponding to the eigenvectors associated with the top $K$ eigenvalues (in absolute value) of $A_{J_l} \in \mathbb{R}^{\abs{J_l} \times \abs{J_l}}$. %\hemant{shouldn't this just be $A_{J_l}$ as defined earlier?}.
The matrix $\hat{U}_{J_l}$ can be transformed to a matrix $\hat{U}^{(l)}$ of size $n\times K$ by completing with 0 
%\hemant{is it NA or $0$? we discussed this before.} 
the rows of the nodes that haven't been observed\footnote{It is easy to verify that $\hat{U}^{(l)}$ is also the eigenvector matrix corresponding to the top $K$ eigenvalues (in absolute value) of $A^{(l)}\odot \Omega^{(l)}$.}. Let $\hat{U}$ be the $n\times KL$ matrix  obtained by stacking $\hat{U}^{(l)}$. 
%\gb{Notation problem fixed, precision about absolute value of eig vect added, and NA replaced by zeros.}

Analogously, let $U_{J_l}$ be the matrix formed by the $K$  eigenvectors corresponding to non-zero eigenvalues of $Z_{J_l}\Pi^{(l)}Z_{J_l}^T$, $U^{(l)}$ be the $n\times K$ matrix obtained from $U_{J_l}$ by filling the rows corresponding to unobserved nodes with the row corresponding to an observed node (belonging to the same community), and
$U$ be the matrix obtained by stacking all the matrices $U^{(l)}$. For each $l$, let $O_l$ be a $K \times K$ orthogonal matrix such that
%
\[ O_l \in \argmin{O^T O=I_k}||\hat{U}_{J_l}-U_{J_l}O ||_F. \]
%
As in the unilayer setting, $k$-means could be applied on the rows of $\hat{U}^{(l)}$ in order to recover the community structure for each $l$. But in order to avoid the label switching problem we propose to apply on the rows of $\hat{U}$ a variant of $k$-means described in \cite{kpod} that can handle missing values, see Algorithm \ref{alg:k-pod}. 
%\hemant{change the sentence ``but as explained..'' as discussed over skype} 
%To avoid this problem, one can  directly perform . However when there are missing values in $\hat{U}$, the $k$-means algorithm can not be applied directly. We overcome this issue by applying an adaptation of Lloyd's algorithm to missing values, namely $k$-pod, studied in~\cite{kpod}. 

Let us describe the principle behind this algorithm. The classical $k$-means problem seeks a partition $Z$ and centroid values (encoded in the matrix $C$) that solves \[ \min_{\substack{Z\in \mathcal{M}_{n,K} \\ C\in \mathbb{R}^{K\times KL}}} ||\hat{U}-ZM ||_F^2 .\] When there are missing values one can instead solve
%
\begin{equation}\label{final:eq1}
    \min_{\substack{Z\in \mathcal{M}_{n,K} \\ C\in \mathbb{R}^{K\times KL}}} ||(\hat{U}-ZM)\odot \maskkpod ||_F^2
\end{equation}   
%
where $\maskkpod = (w^{(1)}\otimes \textbf{1}_K \ \cdots \  w^{(L)}\otimes \textbf{1}_K)$ is the $n\times KL$ mask matrix with
%\hemant{I dont understand the definition of $\maskkpod$ since $\omega_i^{(l)}$ is never defined?} \begin{equation*}
%\gb{I fixed the definition.}
$\textbf{1}_K \in \mathbb{R}^{1 \times K}$ denoting the all ones vector. It is a matrix composed of $L$ blocks where the rows of each block are $1$ if the corresponding node is observed and $0$ otherwise.

\begin{algorithm}[!ht]
\caption{$k$-pod clustering}\label{alg:k-pod}
\begin{flushleft}
        \textbf{Input:} The number of communities $K$, the sets $J_l$ and the adjacency matrices $A_{J_l}$.
\end{flushleft}
\begin{algorithmic}[1]
\State Form $\hat{U}^{(l)}$ from $A_{J_l}$ as explained at the beginning of Section 3.1.
\State Form the matrix $\hat{U}$ by stacking the matrices $\hat{U}^{(l)}$. 
%and initialize $U$ with $\hat{U}$.
\State Initialize the partition $\hat{Z}$ and the centroid matrix $\hat{M}$.

\Repeat
\State  Replace $\hat{U}$ by $\hat{U}\odot \maskkpod + (\hat{Z}\hat{M})\odot (\mathbf{1}\mathbf{1}^T-\maskkpod)$.

\State  Apply $K$-means on the complete matrix $\hat{U}$ and update $\hat{M}$ and $\hat{Z}$.
\Until  convergence.
%
\end{algorithmic}
 \textbf{Output:} A partition of the nodes $\calN =\cup_{i=1}^K \calC_i$ based on $\hat{Z}$.
\end{algorithm}
\gb{In the worst case, the complexity of the algorithm is $O((L+K)n^2)$. But in practice the layers are often sparse and so the complexity will be much less\footnote{This remark regarding the complexity applies to our other methods as well.}.}
%
%
%There is no guarantee that the solution of the above algorithm provides an approximate solution of  \eqref{final:eq1}. However, experiment results in Section \ref{subsec:num_syn_exps} show relatively good performance for this algorithm. 
%The following analysis for the misclustering rate relies on the fact that \eqref{final:eq1} can be (at  least approximately) solved. 
%\hemant{The last sentence is misleading because the next theorem simply gives the misclustering bound for the global solution of \eqref{final:eq1}, isn't it? And \eqref{final:eq1} can always be solved (whether efficiently or not is a different matter, but that is not needed in the proof).}
%
%
\gb{
\begin{theorem}
\label{thm:kpod}
Consider the missing nodes MLSBM in Section \ref{subsec:missing_node_MLSBM}, and suppose that $\rho L\geq 1$, $K L\leq C_0n$, $\rho n_{min}\geq C_1 K^2 \max(\log^2 n, \sqrt{np_{max}})$ and $np_{max}^{(l)}\geq C_2\rho ^{-1}\log n$. 
%for a constant $C_1 > 0$ large enough. 
Let $\lambda_K^{(l)}$ be the $K$-th largest singular value of $\Pi^{(l)}$ and recall that $\beta=n_{max}/n_{min}$. 
%There exist  constants $C_2,C_3, C_4 > 0$ such that 
If \[ \frac{1}{\rho Ln}\sum_l \frac{p_{max}^{(l)}}{(\lambda_K^{(l)})^2} < (30C_3 \beta^4K^3)^{-1}\] then with probability at least $1-O(n^{-1})$, it holds that the solution $\hat{Z} \in \mathcal{M}_{n,K}$ of \eqref{final:eq1} satisfies \[ r(\hat{Z},Z) \leq C_4\exp(-c'\rho L)+\frac{C_5\beta^3K^2}{\rho Ln}\sum_l\frac{p_{max}^{(l)}}{(\lambda_K^{(l)})^2}.\]
\end{theorem}
}
%
The proof of all our theoretical results are deferred to the supplementary material.
%
%\hemant{maybe it should be $p_{max}^{(l)}$ above?}
%\gb{I removed the discussion on the fact that \eqref{final:eq1} is NP hard.}
\begin{remark}
The assumption $\rho L\geq 1$ is natural since $\rho L$ corresponds to the expected total number of times a node is observed, and a node needs to be observed at least once in order to be classified.
The condition $\rho n_{min}\geq C_1 K^2 \log^2 n$ ensures that $\rho$ and $n_{min}$ are not too small. If the communities are well-balanced and the parameters $\rho$ and $K$ are fixed independently of $n$, then the previous condition is satisfied for $n$ large enough.
\end{remark}
%
%
\begin{remark}
Our analysis assumes that each layer is sufficiently informative, and doesn't use the fact that there is more information contained in the whole set of layers than in individual layers. This is why the bound does not improve when $L$ increases. The obtained upper-bound is unlikely to be optimal since as shown in the experiments, the clustering performance does seem to improve a bit when $L$ increases.
\end{remark}



==> Clustering graphs with missing nodes [v2]/preamble.tex <==
%-----------------------------
% Additional packages
%-----------------------------

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amsmath,amssymb,epsfig,amsthm}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{array}
\usepackage{algorithm}
\usepackage{enumerate}
\usepackage{xcolor}
\usepackage{algpseudocode}
\usepackage{xurl}



%-----------------------------
% Theorem like environments
%-----------------------------
\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgment}{Acknowledgment}
\newtheorem{assumption}{Assumption}
\newtheorem{axiom}{Axiom}
\newtheorem{case}{Case}
\newtheorem{claim}{Claim}
\newtheorem{conclusion}{Conclusion}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{criterion}{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}{Solution}
\newtheorem{summary}{Summary}
\numberwithin{equation}{section}




\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\ddiag}{ddiag}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\maximize}{maximize}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\maskkpod}{\Omega_U}
%---------------------------------------------
% Commands for symbols used in the report.
% \mathcal symbols
%----------------------------------------------
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calPp}{\ensuremath{\calP^{\prime}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}




% Miscellaneous symbols 
\newcommand{\tri}{\ensuremath{\bigtriangleup}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\dotprod}[2]{\langle#1,#2\rangle}
\newcommand{\est}[1]{\widehat{#1}}
\newcommand{\expec}{\ensuremath{\mathbb{E}}}
\newcommand{\matR}{\ensuremath{\mathbb{R}}}
\newcommand{\matZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Linfnorm}{L_{\infty}}
\newcommand{\todo}[1]{\textbf{TODO: #1}}
\newcommand{\proj}[2]{\mathcal{R}_{#1}(#2)}
\newcommand{\orproj}{\text{Proj}}
% Comments
\newcommand{\hemant}[1]{\textcolor{red}{HT: #1}}
\newcommand{\gb}[1]{\textcolor{black}{#1}}
\newcommand{\cb}[1]{\textcolor{red}{CB: #1}}

%Indicator variable
\newcommand{\indic}{\ensuremath{\mathbf{1}}} 

% Vectors and matrices
\newcommand{\vecx}{\mathbf x}
\newcommand{\vecn}{\mathbf n}
\newcommand{\vecp}{\mathbf p}
\newcommand{\vecq}{\mathbf q}
\newcommand{\veci}{\mathbf i}
\newcommand{\vecj}{\mathbf j}
\newcommand{\vecu}{\mathbf u}
\newcommand{\vecv}{\mathbf v}
\newcommand{\vecw}{\mathbf w}
\newcommand{\vecb}{\mathbf b}
\newcommand{\vecm}{\mathbf m}
\newcommand{\vecc}{\mathbf c}
\newcommand{\vecy}{\mathbf y}
\newcommand{\vecf}{\mathbf f}
\newcommand{\vecz}{\mathbf z}
\newcommand{\veca}{\mathbf a}
\newcommand{\vecg}{\mathbf g}
\newcommand{\veco}{\mathbf 0}
\newcommand{\matA}{\ensuremath{\mathbf{A}}}
\newcommand{\matB}{\ensuremath{\mathbf{B}}}
\newcommand{\matI}{\ensuremath{\mathbf{I}}}
\newcommand{\matV}{\ensuremath{\mathbf{V}}}
\newcommand{\matH}{\ensuremath{\mathbf{H}}}
\newcommand{\matX}{\ensuremath{\mathbf{X}}}
\newcommand{\matP}{\ensuremath{\mathbf{P}}}

%-------------------
% Paper specific 
%
\newcommand{\kpod}{\texttt{k-pod}}
\newcommand{\sumadjz}{\texttt{sumAdj0}}
\newcommand{\sumadji}{\texttt{sumAdjIter}}
\newcommand{\olmfm}{\texttt{OLMFm}}
\newcommand{\lapla}{\texttt{Laplacian}}
\newcommand{\aggrk}{\texttt{AggrKern}}



==> Clustering graphs with missing nodes [v2]/problem_setup.tex <==
%------------------
% Introduction
%------------------
\section{Problem setup} \label{sec:probsetup}
%
A  multilayer graph is a sequence of graphs $\calG = (\calG ^{(1)}, \ldots , \calG ^{(L)})$. If all the graphs are defined on the same set of nodes $\calN $ indexed by $[n]$, then $\calG$ is said to be pillar. Throughout, we will assume that for all $l\leq L$ each graph $\calG ^{(l)}$ is undirected and has no self-loop. This implies that its associated adjacency matrix $A^{(l)} \in \set{0,1}^{n \times n}$ is symmetric with $A^{(l)}_{ii}=0$ for all $i$. 

Given $\calG$ as input, our goal is to recover a partition of $\calN$ into $K$ disjoint sets (or communities), so that nodes belonging to the same community share a similar connectivity profile. To make the setup more precise, we will study this problem in the setting where $\calG$ is generated via an underlying (unknown) stochastic model, with a latent community structure. This model is a common extension of the well-studied stochastic block model (SBM) for the unilayer case which we now describe.



%----------------
% Unilayer SBM
%-----------------
\subsection{Stochastic Block Model (SBM)}
The stochastic block model (SBM) -- first proposed in \cite{HOLLAND1983109} -- is a simple yet popular stochastic generative model for unilayer graphs which captures the community structures of networks often observed in the real world. 
A SBM with the set of nodes $\calN$ and $K$ communities $\calC_1, \ldots ,\calC_K$ forming a partition of $\calN$ is parameterized as follows. \begin{itemize}
    \item There is a membership matrix $Z \in \calM_{n,K}$ where $\calM_{n,K}$ denotes the class of membership matrices. Here, $Z_{ik}=1$ if node $i$ belongs to $\calC_k$, $0$ otherwise. Each membership matrix $Z$ can be associated bijectively with a function $z:[n]\to [K]$ such that $z(i)=k$ where $k$ is the unique column index satisfying $Z_{ik}=1$.
    \item There is a full-rank, symmetric, connectivity matrix of probabilities $$\Pi=(\pi_{k k'})_{k, k' \in [K]} \in [0,1]^{K \times K}.$$
\end{itemize}
%
%
%
Let us denote $P=(p_{ij})_{i,j \in [n] }:=Z\Pi Z^T$. A graph $\calG$ is distributed according to a stochastic block model SBM$(Z, \Pi)$ if the corresponding symmetric adjacency matrix $A$  has zero diagonal entries and 
%
\[ 
A_{ij}  \overset{\text{ind.}}{\sim} \mathcal{B}(p_{ij}), \quad 1 \leq i < j \leq n,
\] 
%
where $\calB(p)$ denotes a Bernoulli distribution with parameter $p$. Hence the probability that two nodes are connected depends only on the community memberships of these two nodes. 

Let us denote by $n_k$ the size of the community $\calC_k$, $n_{min}$ (resp. $n_{max}$) to be the size of the smallest (resp. largest) community, and $\beta = \frac{n_{max}}{n_{min}}$. The communities are said to be balanced if they all have the same size (equivalently, $\beta=1$). The communities are approximately balanced if $\beta=O(1)$. The maximum value of the connectivity parameter is denoted by $p_{max} := \max_{i,j} p_{ij}$ and can be interpreted as the sparsity level (depending on $n$).

The misclustering rate associated to an estimated membership matrix $\hat{Z}$ is measured by \[ r(\hat{Z},Z)=r(\hat{z},z)=\frac{1}{n}\min _{\sigma \in \mathfrak{S}}\sum_i \indic_{\lbrace \hat{z}(i)\neq \sigma(z(i))\rbrace},\] where $\mathfrak{S}$ denotes the set of permutations on $[K]$. A clustering algorithm is said to be strongly consistent -- or achieving exact recovery -- if $r(\hat{Z},Z)=0$ with probability $1-o(1)$ as $n$ tends to infinity. It is said to be weakly consistent -- or achieving almost exact recovery -- if $\prob(r(\hat{Z},Z)=o(1))=1-o(1)$ as $n$ tends to infinity. A more complete overview of the different types of consistency and the sparsity regimes where they occur can be found in \cite{AbbeSBM}.

%-----------------------
% Multilayer SBM
%-----------------------
\subsection{Multilayer Stochastic Block Model (MLSBM)} \label{subsec:mlsbm}
We now describe the multilayer stochastic block model (MLSBM), which is a common extension of the SBM to the setting of multilayer graphs (see for e.g.,  \cite{paul2020,Bhattacharyya2018SpectralCF, jinLei2019}). The MLSBM is parametrized by the number of layers $L$, a common block membership matrix $Z\in \calM_{n,K}$, and connectivity matrices $\Pi^{(1)}, \ldots, \Pi^{(L)} \in [0,1]^{K \times K}$. 
     
%
%
\paragraph*{}Similar to the unilayer case, let us denote $P^{(l)}=Z\Pi^{(l)}Z^T$ for $l=1,\ldots, L$. A multilayer graph $\calG$ is distributed according to the model MLSBM$(Z, \Pi^{(1)}, \ldots, \Pi^{(L)})$ if the adjacency matrix $A^{(l)}$ of each layer is distributed according to a SBM$(Z,\Pi^{(l)})$ for $l=1,\ldots, L$. Hence, while the probability that two nodes are connected can vary across layers, the block membership of each node remains unchanged. As in the unilayer case we can define the quantities 
%the sparsity parameters 
%
%\begin{equation*}
$p_{max}^{(l)}=\max_{i,j}p_{ij}^{(l)}, \quad  p_{max}=\max_l p_{max}^{(l)}.$
%
%\end{equation*}
%
%
%-----------------------
% Missing nodes
%-----------------------
\subsection{Missing nodes} \label{subsec:missing_node_MLSBM}
The assumption that all the layers share the same set of nodes is quite restrictive since real world multilayer networks are often `non-pillar'. 
%\gb{I added an example of 'non pillar' network}
We propose to deal with such networks by considering nodes present in some layers but not in others as missing.
Let $w_i^{(l)}$ be a binary variable that records the presence of node $i$ in the layer $l$ where $w_i^{(l)}=1$ if node $i$ is observed in layer $l$ and $0$ otherwise. Denoting $w^{(l)} = (w^{(l)}_1, \ldots ,w^{(l)}_n)^T$, let $\Omega^{(l)}=w^{(l)}(w^{(l)})^T$ be the mask matrices and $\Tilde{A}^{(l)}=A^{(l)}\odot \Omega^{(l)}$ for $l\leq L$ where $\odot$ is the usual Hadamard product. Let $J_l$ denote the set of non-missing nodes in  layer $l$ with $n_{J_l} = \abs{J_l}$.
By a slight abuse of notation we will denote by $A_{J_l}$ the matrix $A_{J_l}^{(l)}$. The number of observed nodes in $\calC_k$ will also be denoted by $n_{J_l, k}$. 
%\hemant{Is the definition of $A_{J_l}, Z_{J_l}$ consistent with that defined in notations earlier? Also, in section 3.1, $A_{J_l}^{(l)}$ is considered.}
%\gb{Since the notation $A_J$ is defined in Section 1 there is no need to repeat the definition. I added in the notation section a definition for $Z_J$. So we have just to define $A_{J_l}$ as $A_{J_l}^{(l)}$ here I think.}
%
Throughout, we assume that the missing nodes are generated as $w_i^{(l)}\overset{\text{ind.}}{\sim} \mathcal{B}(\rho)$ for $i=1,\ldots, n.$ 



==> aggregate_spectr.tex <==
\subsection{Aggregate spectral Kernel : the complete case}
This method was proposed in \cite{paul2020} without theoretical guarantees. The principle is the following. For each layer $l$ we compute $\hat{U}_K^{(l)}$ the matrix formed by the eigenvectors of $A^{(l)}$ corresponding to the top $K$ singular values. Then we compute $\Tilde{U}_K$ the matrix formed by the top $K$ eigenvectors of the sum $\sum_l \hat{U}_K^{(l)}(\hat{U}_K^{(l)})^T $ and perform $k$-means on the rows of $\Tilde{U}_K$.
So we compute the best $K$-rank subspace associated with each layer and then find the $K$-rank subspace that is the closest to all these subspaces. A similar approach has been used in the context of distributed PCA \cite{fan2019}.



\subsection{Aggregate spectral Kernel : the missing nodes case}
